Feature Driven and Point Process Approaches for Popularity Prediction

Predicting popularity, or the total volume of information outbreaks, is an important subproblem for understanding collective behavior in networks. Each of the two main types of recent approaches to the problem, feature-driven and generative models, have desired qualities and clear limitations. This paper bridges the gap between these solutions with a new hybrid approach and a new performance benchmark. We model each social cascade with a marked Hawkes self-exciting point process, and estimate the content virality, memory decay, and user influence. We then learn a predictive layer for popularity prediction using a collection of cascade history. To our surprise, Hawkes process with a predictive overlay outperform recent feature-driven and generative approaches on existing tweet data [43] and a new public benchmark on news tweets. We also found that a basic set of user features and event time summary statistics performs competitively in both classification and regression tasks, and that adding point process information to the feature set further improves predictions. From these observations, we argue that future work on popularity prediction should compare across feature-driven and generative modeling approaches in both classification and regression tasks.

==> introduction.v1.tex <==
%!TEX root = paper.tex

\section{Introduction}

The popularity of an item or an entity can be defined as a measure of received attention, aggregated over a large population of individuals.
While individual social preferences have long been the subject of Social Sciences studies~\cite{GaryCharness2002,StevenD.Levitt2007a}, the mechanisms that drive popularity as an aggregate are still poorly understood.
The tastes, preferences and decisions of individuals are not context-independent.
Well-known phenomena such as social influence~\cite{Cialdini2004} or peer pressure~\cite{EugeneKandel1992} might explain why seemingly similar items achieve vastly different popularities.
Moreover, the amount of individual attention for which items compete is limited~\cite{MIR13}, resulting in some items getting popular at the expense of others.
The non-linear interplay of such factors makes popularity appear to have an inherent random component, therefore utterly unpredictable~\cite{Martin2016}.
Despite these difficulties, popularity study is a rising research field.
The main incentive is its marketing application: being able to predict early future popular items.
In addition, the online environment makes it easier to collect data for studying the popularity of a wide range of items, such as consumer products (in online stores), photos, music and video (iTunes, Netflix, Instagram), businesses (Yelp).% etc.

Popularity modeling and popularity prediction approaches can be regroup in two large classes.
In data-driven methods~\cite{Asur2010,CHE14,Martin2016,Pinto2013}
% were mainly data-driven.
a machine learning algorithm is trained on a large dataset of historical data and used to make predictions about future popularity.
%Historically, the approaches for predicting popularity~
An extensive set of features is engineered to describe items,
%They most often rely on engineering an , 
usually based on the content of the item, past similar items and user features.
The early volume of attention received by a given item has been shown to be particularly informative~\cite{Pinto2013,szabo2010}.
However, these approaches are considered to have rather limited prediction performances~\cite{Martin2016} and they have the drawback of functioning as a black-box, not shedding much light on the internal processes that drive popularity.
The second class of approaches are the generative methods~\cite{Ding2015,Shen2014,yu2015micro,Zhao2015}.
These parametrically model one or several social phenomena driving popularity and learn the parameters of the model on historical data or observed activity.
This novel class of approaches exhibit higher prediction accuracy compared to the data-driven methods~\cite{Zhao2015}, but usually have the drawback of becoming overly complicated.
In order to compensate for unaccounted social phenomena which drive the observed popularity away from the theoretical model, some of these methods employ complicated regularization techniques which hinder the interpretability of the generative model.

\textbf{A hybrid approach.}
\TODO{MAR}{Reposition our work as bridging the gap between the two classes, studying for they can be used together to boost prediction performances.
But need results from Hawkes + data-driven}
In this work, we propose a two-step approach towards popularity prediction, which separate modeling the activity on individual items and the relations between items.
\textbf{In the first step}, we model the activity on each item individually, by considering the characteristics of users and the temporal patterns of their interaction with the item.
%
%We design a generative approach towards modeling information diffusion, by employing a 
%
We employ a \emph{Hawkes self-exciting process}~\cite{HAWKES1971} and we design a streamlined, intuitive generative model, which accounts directly for the influence of users over others, the length of ``social memory'' and the inherent item quality.
We mathematically model the following process:
%We use it to model social contagion~\verify{[ref?]}, one of the key factors in information diffusion, and which drives popularity:
when a user interacts with with an item (we denote this as \emph{an event}), not only is the popularity of the item increases, but other users are also exposed to the given item.
Each event spawns new events according to a time-decaying probability and the series of events is modeled as a non-homogeneous Poisson point-process, in which the rate of generation of new events is determined by the past activity.
%The main contribution of our work over alternative generative models~\cite{Crane2008,Zhao2015}\verify{[other refs?]} is 
We infer the parameters of our model using a max-log-likelihood procedure, by observing a prefix of the event series.
While the generative model directly allows to compute the expected total number of events -- i.e. \emph{the total popularity} -- this estimate is made in isolation, without information about other items.
For this reason, \textbf{in the second step} of our approach, we make use of collection-wise information to correct for unseen social phenomena and for connections between items.
We apply a predictive layer on top of the outputs of the individual generative models and we use historical information to train a Random Forrest regressor, which is afterwards used to correct the individual predictions.

\begin{figure}[tbp]
	\includegraphics[width=0.48\textwidth]{spock-dead-cascade-v3}
    \caption{
	Illustration as point processes of two retweet cascades announcing the death of ``Mr. Spock''.
%	$tw_1$ and $tw_2$ are just two of the many retweet cascades related to the NY Times article about the event.
	The underlying diffusion processes of $tw_1$ and $tw_2$ are very different: 
	$tw_1$ attracts the attention of highly influential users, especially music related channels, however the generative kernel of $tw_2$ amplifies more and decays slower than that of $tw_1$.
	The diffusion of $tw_2$ is more dynamic, grows faster and ends in just 12 minutes ($tw_1$ lasts for 2.5 hours), but the final sizes for the two cascades are similar (224 retweets for $tw_1$ and 219 for $tw_2$).
%		unlike $tw_2$ which is tweeted by more regular users.
%	However, the generative kernel of $tw_1$ amplifies less and decays faster than that of $tw_2$ (see inset), leading to 
	We model and interpret these cascades using our generative model in Sec.~\ref{subsec:model-interpretation}.
    }
    \label{fig:example-cascade}
\end{figure}

We apply our model to the task of predicting the popularity of tweets, defined as the total volume of obtained retweets.
We construct a large dataset, containing 49.7 million tweets centered around English news articles, emitted by \TODO{SM}{XXX,000 users} over a period of 6 months, in 2015. 
Fig.~\ref{fig:example-cascade} illustrates as point processes two of the retweet cascades relating the passing away of ``Mr. Spock''.
We show that our approach consistently outperforms the current state-of-the-art generative model~\cite{Zhao2015}, regardless of the length of observed retweet series (\TODO{SM}{give appealing statistic here: e.g. a 30\% increase in accuracy when observing the retweet series for 10 minutes}).
In addition, we build and test a data-driven forecasting system, which employs the most predictive features, highlighted by previous studies: user related features~\cite{Martin2016} and recent activity features~\cite{CHE14}.
We show that our proposed hybrid generative-predictive system consistently outperforms the data-driven predictor, both in a classification task -- \verify{XX\% \TODO{SM}{appealing statistic here}} -- and in a regression task -- accuracy improves by \verify{XX\% \TODO{SM}{fill this in}}.

\textbf{Main contributions.} 
Our work makes several contributions, as follows:
\squishlisttwo
	\item \textbf{Model:} the paper proposes a hybrid popularity prediction system, made of two components: i) an intuitive, streamlined generative model for the attention series, with design choices based on social phenomena and trained individually for each item and ii) a predictive layer accounting for collection-wise information and items interactions;
	\item \textbf{Dataset:} we construct and curate a large dataset of retweet diffusion cascades, which will be made available to the community\footnote{Twitter API user agreement requires user ids annonimyzation prior to publication.} as a benchmark. The current benchmark dataset~\cite{Zhao2015} lacks user information, making it impossible to leverage such information.
	\item \textbf{Prediction perfomances:} we perform extensive experiments, on two large datasets, showing that our proposed popularity prediction approach consistently outperforms both the current state of the art generative and data-driven models.
\squishend

The rest of this paper is structured as follows.
Sec.~\ref{sec:related-work} presents some prior related work.
Sec.~\ref{sec:model} details the proposed generative model and fitting methods, while Sec.~\ref{sec:prediction} presents how the popularity prediction is performed, based on the fitted model parameters.
The dataset and the experiments comparing our model to the state-of-the-art baselines are outlined in Sec.~\ref{sec:xp} and we conclude in Sec.~\ref{sec:conclusion}.

%we setup two experiments to evaluate the explanatory power of our model.
%When exploring the limits of predictability of popularity, Martin \etal~\cite{Martin2016} theorize that considerable amounts of new information is required to go beyond what can be predicted using data-driven approaches.
%In the first experiment, we show that by observing the same amount of information (the first 5 minutes of retweeting series), our model achieves improved prediction results, thus showing that it is capable of capturing more information about the cascade than a traditional classifier.
%In the second experiment, we evaluate the predictive power of our model's parameters.
%Using the same experimental setup as in Cheng \etal~\cite{CHE14}, we employ the learned values of our model's parameters as features in a binary classifier, aiming at predicting if a given cascade will double its current size.
%We show that the prediction accuracy improves by \verify{XX\% \TODO{SM}{fill this in}}, over a data-driven model containing the features shown as most predictive in~\cite{CHE14}: recent activity and user influence features.
%This shows that our generative model accounts better for the non-linear interplay between past event times and user influence.

%%Basically we want to give following as our contribution:
%\rev{Main contributions/messages to pass through:}
%\begin{itemize}
%	\item simple, \rev{elegant} model;
%	\item \rev{generative model, i.e. parameters are interpretable}
%	\item clearer inference and estimation
%	\item beats state of art generative model \rev{in the task of final star volume prediction} 
%	\item say unlike Cheng \etal only some features can do better prediction, just change what you are looking for \TODO{SM}{This does not read}
%	\item \rev{our model better accounts for non-linear temporal relations: using the same information as~\cite{CHE14}, we use our models parameters as features in a classification setting and predict}
%	%model can be adopted for another setting(classification) and do predictions concerning 
%	the continuous growth of cascades. 
%\end{itemize}

==> introduction.v2.tex <==
%!TEX root = paper.tex

\newpage
\section{Introduction}

Popularity prediction, especially in the context of online media, has seen increased attention, as
%has been a very active research field.
%The main incentive is its marketing application: the early prediction of future popular items.
successful solutions would help both content consumers to cope with information overload, and content producers to disseminate information within limited resources.
%The great wealth of approaches proposed in recent years %%LX: drop the drama
%
% MAR: refocus discussion
When presented with the task of predicting popularity in a specific application, a clear gap appears concerning available methods:
\emph{feature-driven approaches}~\cite{Asur2010,CHE14,Martin2016,Pinto2013} engineer an extensive set of features, which are usually course information summaries about the content or the user characteristics;
\emph{generative methods}~\cite{Ding2015,Shen2014,yu2015micro,Zhao2015} leverage the fine-grained information in the event series, however they make stronger assumptions about the diffusion process.
A thorough comparison of the predictive performances of the two classes is currently missing, especially since the generative methods are usually designed for explaining the mechanisms that generate attention, and not optimized for predicting.
Furthermore, for the feature-driven approaches, there is no consensus about a set of features which are simultaneously informative for popularity and do not require comprehensive or restrictive access to the data source (like private user information or measurements over the entire diffusion network).
Neither is it clear which features generalize well across different learning tasks, including: 
predicting the volume of attention~\cite{Shen2014,Zhao2015}, 
predicting if a retweet cascade will double in size~\cite{CHE14}, 
whether an item will have 10 million views~\cite{shamma2011viral}, or be among the top 5\% most popular~\cite{yu2014twitter}.

%Recent approaches address popularity prediction with a variety of methods, learning tasks and datasets. 
%However when one is presented with the task of predicting popularity in a specific application, unanswered questions arise:
%does modeling popularity through generative processes yield better prediction performances than feature-based approaches?
%%constructing expressive features and feeding them into a machine learning predictor?
%which of the conclusions reported on datasets rich in restricted insider information are maintained for domains specific, free access datasets?
%%
%For example, feature-driven methods~\cite{Asur2010,CHE14,Martin2016,Pinto2013} engineer an extensive set of features, usually based on content and user characteristics, used together with a machine learning algorithm to make predictions about future popularity.
%However, such approaches most often require specialized information which might not be available with other data sources, like private user information or measurements over the entire diffusion network.
%For this reason, there is no consensus about a set of features which are simultaneously informative for popularity and do not require comprehensive or restrictive access to the data source.
%Neither is it clear which features generalize well across different learning tasks, including: 
%predicting the volume of attention~\cite{Shen2014,Zhao2015}, 
%predicting if a retweet cascade will double in size~\cite{CHE14}, 
%whether an item will have 10 million views~\cite{shamma2011viral}, or be among the top 5\% most popular~\cite{yu2014twitter}.

%In this work, we address the above questions by proposing several contributions.
In this paper, we setup to the task of bridging the gap between the two broad classes of approaches, and we show results applied to predicting the final size of retweet cascades.
We build two novel predictive approaches, one from each class, and we show how to combine them into a hybrid predictor to further increase performances.
The generative method is a two-layered approach, built on the intuitive \emph{Hawkes self-exciting process}~\cite{HAWKES1971} model.
Self-exciting point processes are a class of stochastic processes, in which the occurrence of past events makes the occurrence of future events more probable.
Three key factors in information diffusion are built into the proposed model: the social influence of users, the length of ``social memory'' and the inherent tweet quality.
We fit the model parameters for each cascade individually by maximizing data likelihood on the initial unfolding of the cascade.
The generative model allows a direct estimation of the total number of events -- i.e. \emph{the total popularity} -- however, this estimate is made in isolation, without information about other cascades.
We correct individual model predictions by systematically constructing a predictive layer on top of the model parameters.
In addition to predicting final popularity more accurate than the current state-of-the-art, this method captures characteristics of individual cascades (for example, the speed at which events unfold) or collections of cascades.
Our second proposed approach, the feature-based method, uses
%For the latter, we select and construct 
only features which can be computed solely on data provided by free access APIs and which were highlighted as most predictive by recent studies: user related features~\cite{Martin2016} and temporal activity features~\cite{CHE14}.
This results in a surprisingly competitive feature-based predictor, which consistently outperforms the current state-of-the-art popularity prediction model~\cite{Zhao2015} -- reducing the mean absolute relative error by more than 200\%, after observing the retweet series for 10 minutes.
We show that the same set of features can be employed in both regression and classification tasks.
We further experiment with a hybrid predictor, which uses both data features and measures issued from the generative model,
%either by introducing data features are also used in the predictive layer, 
and we show additional performance improvement.
%
%
%We show the resulted system to consistently outperform the current state-of-the-art in estimating final cascade sizes.
%The resulted prediction system outperforms both the state-of-the-art and our previously proposed feature-driven approach when 
%
%
%%Firstly, we bridge the gap in the problem space of predicting popularity using feature-driven approaches.
%We 
%
%Our second contribution is a two-layered generative approach to popularity prediction.
%%Generative methods~\cite{Ding2015,Shen2014,yu2015micro,Zhao2015} 
%%%rely on mathematically modeling the sames 
%%aims to explain the mechanism that generates attention, but are not optimized for prediction.
%%rather than learning from context.
%We build on the intuitive %design a streamlined, intuitive 
%\emph{Hawkes self-exciting process}~\cite{HAWKES1971} model, which accounts directly for three key factors in information diffusion: the social influence of users, the length of ``social memory'' and the inherent tweet quality.
%%
%%
%%We model the activity on each item individually, by considering the characteristics of users and the temporal patterns of their interaction with the item.
%%%
%%%We design a generative approach towards modeling information diffusion, by employing a 
%%%
%%We employ a \emph{Hawkes self-exciting process}~\cite{HAWKES1971} and we design a streamlined, intuitive generative model, which accounts directly for the influence of users over others, the length of ``social memory'' and the inherent item quality.
%We mathematically model the following process:
%%when a user retweets (we denote this as \emph{an event}), 
%%not only she increases the popularity of the initial tweet, %%LX: what does this mean?!
%%but she also exposes other users to the tweet.
%each (tweeting) event spawns other new events according to a time-decaying probability. 
%The series of events is modeled as a non-homogeneous Poisson point-process, in which the rate of arrival of new events is determined by the past activity.
%We fit the model parameters for each cascade individually by maximizing data likelihood. 
%%procedure, to allow a flexible description of the diffusion process.
%%We infer the parameters of our model using a max-log-likelihood procedure, by observing a prefix of the event series.
%The generative model allows a direct estimation of the total number of events -- i.e. \emph{the total popularity} -- however, this estimate is made in isolation, without information about other cascades.
%We systematically construct a predictive layer on top of the model parameters, which corrects the individual model predictions.
%The resulted prediction system outperforms both the state-of-the-art and our previously proposed feature-driven approach when estimating final cascade sizes.
%We further experiment with a hybrid approach, in which data features are also used in the predictive layer, and we show additional performance improvement.
%
%For this reason, \textbf{in the second step} of our approach, we make use of collection-wise information to correct for unseen social phenomena and for connections between items.
%We apply a predictive layer on top of the outputs of the individual generative models and we use historical information to train a Random Forrest regressor, which is afterwards used to correct the individual predictions.
%
\begin{figure}[tbp]
	\includegraphics[width=0.48\textwidth]{spock-dead-cascade-v3}
    \caption{
	Illustration as point processes of two retweet cascades announcing the death of ``Mr. Spock''.
%	$tw_1$ and $tw_2$ are just two of the many retweet cascades related to the NY Times article about the event.
	The underlying diffusion processes of $tw_1$ and $tw_2$ are very different: 
	$tw_1$ lasts for 2.5 hours. It attracts the attention of highly influential users, especially music related channels, however the generative kernel of $tw_2$ amplifies more than that of $tw_1$.
	%The diffusion of $tw_2$ is more dynamic, grows %%LX: not clear what "dynamic" means as an adjective!
	$tw_2$ diffuses	faster and ends in just 12 minutes, but the final sizes for the two cascades are similar (224 retweets for $tw_1$ and 219 for $tw_2$).
%		unlike $tw_2$ which is tweeted by more regular users.
%	However, the generative kernel of $tw_1$ amplifies less and decays faster than that of $tw_2$ (see inset), leading to 
	We model and interpret these cascades using our generative model in Sec.~\ref{subsec:model-interpretation}.
	x-axis: time in seconds; y-axis: number of followers each tweet can reach; $\phi_m(\tau)$: memory kernel of Eq.~\eqref{eq:phi-separable} plotted with $m=1000$. 
    }
    \label{fig:example-cascade}\captionmoveup
\end{figure}
%
%We apply our model to the task of predicting the popularity of tweets, defined as the total volume of obtained retweets.
We conduct experiments on a large dataset, containing 49.7 million tweets about English news articles, gathered using the public API over a period of 4 months, in 2015. 
Fig.~\ref{fig:example-cascade} illustrates as point processes two of the retweet cascades in this dataset, relating the passing of the actor for ``Mr. Spock''.
Even though the two cascades achieve similar popularities, our generative model is capable of differentiating between their very different diffusion dynamics.
For example, the memory kernel $\phi_m(\tau)$ of $tw_2$ -- i.e. the contribution of each event to the spawning of future events -- shows a large total amplification, but a short social memory.

%We show that our approach consistently outperforms the current state-of-the-art generative model~\cite{Zhao2015}, regardless of the length of observed retweet series (\TODO{SM}{give appealing statistic here: e.g. a 30\% increase in accuracy when observing the retweet series for 10 minutes}).
%In addition, we build and test a data-driven forecasting system, which employs the most predictive features, highlighted by previous studies: user related features~\cite{Martin2016} and recent activity features~\cite{CHE14}.
%We show that our proposed hybrid generative-predictive system consistently outperforms the data-driven predictor, both in a classification task -- \verify{XX\% \TODO{SM}{appealing statistic here}} -- and in a regression task -- accuracy improves by \verify{XX\% \TODO{SM}{fill this in}}.

%\newpage
There are three main contributions of this paper:
\squishlisttwo
	\item \textbf{Bridging the popularity prediction problem space:} 
	we compare approaches to popularity prediction from the two main classes, i.e. feature-based and generative, and we show that combining them into a hybrid approach increases performances;
	we identify a set of informative features, which can be constructed using data gathered through free access APIs and usable for both regression and classification tasks.
%	we build a competitive feature-based predictor, with good performances when predicting both the volume of retweet cascades (regression) and whether a cascade will double in size (classification);
%	we compare the feature-driven approach with generative approaches on two large datasets and we show it to consistently outperform the current state of the art generative method~\cite{Zhao2015}.
	
	\item \textbf{Predicting popularity with generative models:} 
	we propose a generative method, based on Hawkes self-exciting processes, which features the advantages of generative methods -- e.g. interpretable results -- and which is adapted for predicting the final cascade popularity by using an additional predictive layer.
%	 account for the three key ingredients in diffusion in social media;
%	we systematically construct a predictive layer on top of the generative method, which outperforms both the feature-based predictor and the state-of-the-art;
%	we find that fitting the model's parameters for each cascade ensures full flexibility for the three dimensions of the diffusion, which accounts for both better interpretability and predictability.
%	the paper proposes a hybrid popularity prediction system, made of two components: i) an intuitive, streamlined generative model for the attention series, with design choices based on social phenomena and trained individually for each item and ii) a predictive layer accounting for collection-wise information and items interactions;

	\item \textbf{Dataset:} we construct and curate a large, domain-specific dataset of retweet diffusion cascades, which together with the code to fit the generative model, is publicly available for download.\footnote{Download data and code here: \url{https://git.io/v6rIN}.} 
%after appropriate anonymization. 
%The current benchmark dataset~\cite{Zhao2015} lacks user information, making it impossible to test feature-based approaches.
	This new dataset allows comprehensive performance benchmarks on features about users and temporal activity.
%	\item \textbf{Prediction perfomances:} we perform extensive experiments, on two large datasets, showing that our proposed popularity prediction approach consistently outperforms both the current state of the art generative and data-driven models.
\squishend

% removing plan of paper, never quite got it anyways
The rest of this paper is structured as follows.
Sec.~\ref{sec:related-work} presents related work.
Sec.~\ref{sec:model} details the proposed generative model and fitting methods, while Sec.~\ref{sec:prediction} presents how the popularity prediction is performed, based on the fitted model parameters.
The dataset and feature construction for the feature-driven approach are detailed in Sec.~\ref{sec:data} and the experiments are outlined in Sec.~\ref{sec:xp}.
We conclude in Sec.~\ref{sec:conclusion}.





%%%%%%%%%%%%%%%%%%%%%%%%%%% FROM HERE OLD AND USELESS

%we setup two experiments to evaluate the explanatory power of our model.
%When exploring the limits of predictability of popularity, Martin \etal~\cite{Martin2016} theorize that considerable amounts of new information is required to go beyond what can be predicted using data-driven approaches.
%In the first experiment, we show that by observing the same amount of information (the first 5 minutes of retweeting series), our model achieves improved prediction results, thus showing that it is capable of capturing more information about the cascade than a traditional classifier.
%In the second experiment, we evaluate the predictive power of our model's parameters.
%Using the same experimental setup as in Cheng \etal~\cite{CHE14}, we employ the learned values of our model's parameters as features in a binary classifier, aiming at predicting if a given cascade will double its current size.
%We show that the prediction accuracy improves by \verify{XX\% \TODO{SM}{fill this in}}, over a data-driven model containing the features shown as most predictive in~\cite{CHE14}: recent activity and user influence features.
%This shows that our generative model accounts better for the non-linear interplay between past event times and user influence.

%%Basically we want to give following as our contribution:
%\rev{Main contributions/messages to pass through:}
%\begin{itemize}
%	\item simple, \rev{elegant} model;
%	\item \rev{generative model, i.e. parameters are interpretable}
%	\item clearer inference and estimation
%	\item beats state of art generative model \rev{in the task of final star volume prediction} 
%	\item say unlike Cheng \etal only some features can do better prediction, just change what you are looking for \TODO{SM}{This does not read}
%	\item \rev{our model better accounts for non-linear temporal relations: using the same information as~\cite{CHE14}, we use our models parameters as features in a classification setting and predict}
%	%model can be adopted for another setting(classification) and do predictions concerning 
%	the continuous growth of cascades. 
%\end{itemize}

%%%%%%%%%%%%%%%%%%% FROM OLD INTRO
%The popularity of an item or an entity can be defined as a measure of received attention, aggregated over a large population of individuals.
%While individual social preferences have long been the subject of Social Sciences studies~\cite{GaryCharness2002,StevenD.Levitt2007a}, the mechanisms that drive popularity as an aggregate are still poorly understood.
%The tastes, preferences and decisions of individuals are not context-independent.
%Well-known phenomena such as social influence~\cite{Cialdini2004} or peer pressure~\cite{EugeneKandel1992} might explain why seemingly similar items achieve vastly different popularities.
%Moreover, the amount of individual attention for which items compete is limited~\cite{MIR13}, resulting in some items getting popular at the expense of others.
%The non-linear interplay of such factors makes popularity appear to have an inherent random component, therefore utterly unpredictable~\cite{Martin2016}.
%Despite these difficulties, popularity study is a rising research field.
%The main incentive is its marketing application: being able to predict early future popular items.
%In addition, the online environment makes it easier to collect data for studying the popularity of a wide range of items, such as consumer products (in online stores), photos, music and video (iTunes, Netflix, Instagram), businesses (Yelp).% etc.
%
%Popularity modeling and popularity prediction approaches can be regroup in two large classes.
%In data-driven methods~\cite{Asur2010,CHE14,Martin2016,Pinto2013}
%% were mainly data-driven.
%a machine learning algorithm is trained on a large dataset of historical data and used to make predictions about future popularity.
%%Historically, the approaches for predicting popularity~
%An extensive set of features is engineered to describe items,
%%They most often rely on engineering an , 
%usually based on the content of the item, past similar items and user features.
%The early volume of attention received by a given item has been shown to be particularly informative~\cite{Pinto2013,szabo2010}.
%However, these approaches are considered to have rather limited prediction performances~\cite{Martin2016} and they have the drawback of functioning as a black-box, not shedding much light on the internal processes that drive popularity.
%The second class of approaches are the generative methods~\cite{Ding2015,Shen2014,yu2015micro,Zhao2015}.
%These parametrically model one or several social phenomena driving popularity and learn the parameters of the model on historical data or observed activity.
%This novel class of approaches exhibit higher prediction accuracy compared to the data-driven methods~\cite{Zhao2015}, but usually have the drawback of becoming overly complicated.
%In order to compensate for unaccounted social phenomena which drive the observed popularity away from the theoretical model, some of these methods employ complicated regularization techniques which hinder the interpretability of the generative model.
